QAL-BP: An Augmented Lagrangian Quantum Approach for Bin Packing

The bin packing is a well-known NP-Hard problem in the domain of artificial intelligence, posing significant challenges in finding efficient solutions. Conversely, recent advancements in quantum technologies have shown promising potential for achieving substantial computational speedup, particularly in certain problem classes, such as combinatorial optimization. In this study, we introduce QAL-BP, a novel Quadratic Unconstrained Binary Optimization (QUBO) formulation designed specifically for bin packing and suitable for quantum computation. QAL-BP utilizes the Augmented Lagrangian method to incorporate the bin packing constraints into the objective function while also facilitating an analytical estimation of heuristic, but empirically robust, penalty multipliers. This approach leads to a more versatile and generalizable model that eliminates the need for empirically calculating instance-dependent Lagrangian coefficients, a requirement commonly encountered in alternative QUBO formulations for similar problems. To assess the effectiveness of our proposed approach, we conduct experiments on a set of bin packing instances using a real Quantum Annealing device. Additionally, we compare the results with those obtained from two different classical solvers, namely simulated annealing and Gurobi. The experimental findings not only confirm the correctness of the proposed formulation but also demonstrate the potential of quantum computation in effectively solving the bin packing problem, particularly as more reliable quantum technology becomes available.

==> guidlines.tex <==
Introduction
The Introduction section, of referenced text expands on the background of the work (some overlap with the Abstract is
acceptable). The introduction should not include subheadings.
-------------------------------------------------------------
Results
Up to three levels of subheading are permitted. Subheadings should not be numbered.

Subsection
Example text under a subsection. Bulleted lists may be used where appropriate, e.g.
• First item
• Second item

Third-level section
Topical subheadings are allowed.
-------------------------------------------------------------

Discussion
The Discussion should be succinct and must not contain subheadings.

-------------------------------------------------------------

Methods
Topical subheadings are allowed. Authors must ensure that their Methods section includes adequate experimental and
characterization data necessary for others in the field to reproduce their work.
